ProDiff: Progressive Fast Diffusion Model For High-Quality Text-to-Speech

Denoising diffusion probabilistic models (DDPMs) have recently achieved leading performances in many generative tasks. However, the inherited iterative sampling process costs hinder their applications to text-to-speech deployment. Through the preliminary study on diffusion model parameterization, we find that previous gradient-based TTS models require hundreds or thousands of iterations to guarantee high sample quality, which poses a challenge for accelerating sampling. In this work, we propose ProDiff, on progressive fast diffusion model for high-quality text-to-speech. Unlike previous work estimating the gradient for data density, ProDiff parameterizes the denoising model by directly predicting clean data to avoid distinct quality degradation in accelerating sampling. To tackle the model convergence challenge with decreased diffusion iterations, ProDiff reduces the data variance in the target site via knowledge distillation. Specifically, the denoising model uses the generated mel-spectrogram from an N-step DDIM teacher as the training target and distills the behavior into a new model with N/2 steps. As such, it allows the TTS model to make sharp predictions and further reduces the sampling time by orders of magnitude. Our evaluation demonstrates that ProDiff needs only 2 iterations to synthesize high-fidelity mel-spectrograms, while it maintains sample quality and diversity competitive with state-of-the-art models using hundreds of steps. ProDiff enables a sampling speed of 24x faster than real-time on a single NVIDIA 2080Ti GPU, making diffusion models practically applicable to text-to-speech synthesis deployment for the first time. Our extensive ablation studies demonstrate that each design in ProDiff is effective, and we further show that ProDiff can be easily extended to the multi-speaker setting. Audio samples are available at \url{https://ProDiff.github.io/.}

==> sections/old.tex <==
\subsection{Adversarial learning}

In ProDiff, we parameterize the denoising model by $p_\theta(\vx_{t-1}|\vx_t) := q(\vx_{t-1}|\vx_t,\vx_0=f_{\theta}(\vx_t|t,c))$. Since conditional GANs with adversarial learning~\cite{yang2021ganspeech,min2021meta} have been shown to model complex conditional distributions in speech synthesis, we adopt them to approximate the true denoising distribution $q\left(\vx_{t-1}|\vx_{t}\right)$. Our training is formulated by matching the conditional GAN generator $p_{\theta}(\vx_{t-1}|\vx_{t})$ and $q(\vx_{t-1}|\vx_{t})$ using an adversarial loss that minimizes a divergence $D_{\mathrm{adv}}$ per denoising step:

\begin{equation}
    \min _{\theta} \sum_{t \geq 1} \mathbb{E}_{q(t)}[D_{\mathrm{adv}}(q(\vx_{t-1}|\vx_{t}) \| p_{\theta}(\vx_{t-1}|\vx_{t}))]
\end{equation}

where $D_{\mathrm{adv}}$ can be Wasserstein distance, Jenson-Shannon divergence, or f-divergence depending on the adversarial training setup. 

To set up the adversarial training, we denote the conditional time-dependent discriminator as $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c)$ with parameters $\phi$. It takes the N-dimensional $\vx_{t-1}$ and $\vx_{t}$ as inputs, and decides whether $\vx_{t-1}$ is a plausible denoised version of $\vx_{t}$ conditioned on intermediate features $c$. We use the least-squares loss~\cite{mao2017least} for adversarial training:
\begin{align} ~\label{eq: discriminator}
    \begin{split}
    \min _{\phi} \sum_{t \geq 1} \mathbb{E}_{q(\vx_{t})}[\mathbb{E}_{q(\vx_{t-1}|\vx_{t})}[(D_{\phi}(\vx_{t-1}, \vx_{t}, t, c) - 1)^2] \\+\mathbb{E}_{p_{\theta}(\vx_{t-1}|\vx_{t})}[D_{\phi}(\vx_{t-1}, \vx_{t}, t, c)^2],
\end{split}
\end{align}

where fake samples from $p_{\theta}(\vx_{t-1}|\vx_{t})$ are contrasted against real samples from $q(\vx_{t-1}|\vx_{t})$.

Given the discriminator, we updates the generator with following GAN objective:
\begin{equation} \label{eq: generator}
\min _{\theta} \sum_{t>1} \mathbb{E}_{q(\vx_{t})} \mathbb{E}_{p_{\theta}(\vx_{t-1}|\vx_{t})}[(D_{\phi}(\vx_{t-1}, \vx_{t}, t, c) - 1)^2]
\end{equation}


\subsection{Motivation}
Previous diffusion models~\cite{jeong2021diff,liu2021diffsinger} mainly utilize the simple loss objective (e.g., MSE or MAE) to reconstruct acoustic features. However, this optimization is demonstrated~\cite{ren2022revisiting,liu2021diffsinger} to be based on the incorrect unimodal distribution assumptions, leading to blurry and oversmoothing predictions in mel-spectrograms.

2) ProDiff adopts the adversarial training method to prevent the over-smooth issues in generated samples. Generative adversarial networks~\cite{goodfellow2014generative} with competitive games assist to model the dependent and multimodal distribution~\cite{ren2022revisiting,yang2021ganspeech}, which equip ProDiff with ablity to generate samples of high perceptual quality.


\subsection{Architecture}
4) adversarial loss $\gL_{adv}$: the GAN objectives with conditional time-dependent discriminators to minimize a divergence $D_{\mathrm{adv}}$ per denoising step; 


The spectrogram discriminator, $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c=\text{mel})$, takes ground-truth mel spectrograms as input, and measure the similarity of distribution between generated and real acoustic features as well as consider whether the generated samples match the input spectrogram. It adopts multiple random window discriminators (MWRDs)~\cite{wu2020adversarially} with random window sizes which are independent of each other. In addition, the random window sizes in MRWDs have been demonstrated for its efficiency in reducing the computational complexity in training.

The phoneme discriminator, $D_{\phi}(\vx_{t-1}, \vx_{t}, t, c=\text{phoneme})$, takes phoneme sequences as input, and distinguishes the real speech from the generated speech given the phoneme sequence tq as the condition. In particular, the phoneme discriminator consists of fully-connected layers and is applied at frame level. Since we know the duration of each phoneme, we can concatenate each frame in mel-spectrogram with the corresponding phoneme. The discriminator then computes scalars for each frame and averages them to get a single scalar.

\subsection{Related work}

\subsection{Adversarial learning}
Adversarial learning has showed powerful performance in several image domains~\cite{wang2018high,zhang2018stackgan++}, and is adopted successfully in speech domain. GAN-based neural vocoders~\cite{kong2020hifi,kumar2019melgan} show comparable performance to the autoregressive state-of-the-art model and can synthesize speech in real-time. Researchers~\cite{donahue2020end} found that an important advantage of adversarial losses for TTS is a focus on realism over diversity, which enables a more efficient use of capacity compared to models trained with maximum likelihood. Different from previous work, we adopts the adversarial training method to prevent the over-smooth issues in generated samples.
